Why Generalization in RL is Difficult: Epistemic POMDPs and Implicit Partial Observability

Generalization is a central challenge for the deployment of reinforcement learning (RL) systems in the real world. In this paper, we show that the sequential structure of the RL problem necessitates new approaches to generalization beyond the well-studied techniques used in supervised learning. While supervised learning methods can generalize effectively without explicitly accounting for epistemic uncertainty, we show that, perhaps surprisingly, this is not the case in RL. We show that generalization to unseen test conditions from a limited number of training conditions induces implicit partial observability, effectively turning even fully-observed MDPs into POMDPs. Informed by this observation, we recast the problem of generalization in RL as solving the induced partially observed Markov decision process, which we call the epistemic POMDP. We demonstrate the failure modes of algorithms that do not appropriately handle this partial observability, and suggest a simple ensemble-based technique for approximately solving the partially observed problem. Empirically, we demonstrate that our simple algorithm derived from the epistemic POMDP achieves significant gains in generalization over current methods on the Procgen benchmark suite.

==> intro_rewrite.tex <==

Generalization is a central challenge in machine learning. However, much of the research on reinforcement learning (RL) has been concerned with the problem of optimization: how to master a specific task through online or logged interaction. Generalization to new test-time scenarios has received comparatively less attention, although several works have observed empirically \citep{?} that generalization poses a significant challenge to policies trained with RL. In standard supervised learning, it is known that in the absence of distribution shift, optimizing for performance on the training set (i.e., empirical risk minimization) translates into good generalization performance, and it is tempting to suppose that the generalization challenges in RL can be solved in the same way.

In this paper, we will show that this is not the case, and that the structure of the RL problem setting requires designing novel strategies distinct from those in supervised learning. For example, while a classification model seeking to maximize predictive accuracy can simply output the label it considers most likely, regardless of its confidence about this prediction, an RL agent cannot do the same. Since the reward function induces a potentially non-uniform risk profile, to act optimally, an agent must rather factor in this uncertainty to balance between executing conservative behaviors with mediocre payoffs and high-risk behaviors with potentially high payoffs. Further, while supervised learning models receive no feedback during test-time, RL agents are evaluated in a feedback loop that can be leveraged to increase test-time return, whether by switching strategies when it becomes clear the previous strategy is not working, or by proactively taking epistemic actions to determine which strategy to pursue in this new scenario.

As an anecdotal example of how these factors affect , imagine a robotic zookeeper for feeding otters. After being trained in many zoos, the robot is deployed in a new zoo, where it finds that it is uncertain about which door leads to the otter enclosure and which to the tiger enclosure (entering the tiger enclosure leads to low reward for the robot, but amuses the tigers). In the agent's observation contains 
The agent's observation vector contains an image of a map of the zoo, and the optimal policy in the underlying environment parses this map from pixels to perfectly identify the otter enclosure and enter the habitat. However, a policy \textit{learned} from the limited set of training zoos that mimics this strategy (trying to parse the pixels of the map to ascertain the identity of the otter enclosure) is sub-optimal, since it exposes the agent to high regret if the agent's network fails to generalize to any of the new map images at evaluation time.
An agent that instead peeks through the windows of the habitats (or performs some other epistemic action) to more confidently avoid this high-risk outcome will achieve higher return on average.

While the example described above superficially resembles poor generalization in typical supervised learning settings and might imply that well-studied techniques for inducing generalization in supervised learning may be sufficient in RL, we show that the long-term structure of the RL problem setting requires designing novel strategies distinct from supervised learning. Not only does the long-term structure of RL complicate the strategies for generalization, but the potentially non-uniform risk profiles in RL require the agent to carefully balance more conservative behaviors with mediocre payoffs and behaviors with potentially high payoffs and high risk.
In addition, since the agent's action can affect the state of the environment at the next step, policies that exploit this property by conditioning their behavior based on the observations seen previously in the trajectory can potentially outperform agents that only rely on fixed modes of behavior (as with the zookeeper). These features, amongst others, make standard approaches for generalization sub-optimal in the RL setting, and introduce the need for alternative approaches that factor the structure of the RL problem when optimizing for generalization. 


How can we succinctly describe the set of behaviors needed for a policy to generalize in the RL setting? We make the observation that, even in a fully-observable environment, the agent's epistemic uncertainty renders the environment \textit{implicitly} partially observed at test-time.
In the anecdote, although the image of the map could have been used to locate the otter enclosure had the agent seen a greater number of zoos during training time, the agent cannot reliably learn to parse the map from its small set of training zoos, so the location of the otter enclosure is implicitly obfuscated from the agent. Peeking through the enclosure door provides a more reliable cue for a policy with non-negligible generalization error, even though it would never be necessary for the optimal policy. We formalize this observation, and show that generalizing optimally at test time corresponds to solving a partially-observed process that we call an \textbf{epistemic POMDP}, which is induced by the agent's epistemic uncertainty about the environment. The epistemic POMDP establishes a connection between the problem of generalization in RL and the Bayesian RL framework, where a wide body of work has studied techniques for efficient exploration in online RL during training \citep{addsomebayesianreferences}. 

The epistemic POMDP provides an avenue for understanding how the long-term structure of the RL problem affects the strategies needed to generalize appropriately. The potentially non-uniform risk profiles in RL require the agent to carefully balance between executing conservative behaviors with mediocre payoffs, 
Not only does solving the epistemic POMDP emerge as a principled approach to learn policies, this observation also sheds light on why previously proposed regularizations that heuristically introduce some form of partial observability have performed well empirically. 
We present a algorithm that uses an ensemble of (value functions / policies / TBD) find an approximate solution that uses an ensemble of value functions policies to . Add more discussion about the methods we consider here.






The primary contribution of this paper is a reframing of generalization in RL as the problem of solving a partially observed process, which we call the epistemic POMDP. The epistemic POMDP highlights the additional challenges needed for optimal generalization in RL, as compared to supervised learning. We show both theoretically and empirically the necessity of reasoning about this partial observability in order to maximize test-time performance, and suggest simple methods based on the POMDP formulation for doing so. Our work highlights the importance of not only finding ways to help neural networks in RL generalize better, but also on learning policies that degrade gracefully when the underlying neural network eventually does fail to generalize. Empirically, we demonstrate that algorithms derived from the epistemic POMDP achieve significant gains in performance over current methods on several image-based problems and ProcGen benchmark tasks.


